Optimal Scheduling of Agents in ADTrees: Specialised Algorithm and Declarative Models

Expressing attack-defence trees in a multi-agent setting allows for studying a new aspect of security scenarios, namely how the number of agents and their task assignment impact the performance, e.g. attack time, of strategies executed by opposing coalitions. Optimal scheduling of agents' actions, a non-trivial problem, is thus vital. We discuss associated caveats and propose an algorithm that synthesises such an assignment, targeting minimal attack time and using the minimal number of agents for a given attack-defence tree. We also investigate an alternative approach for the same problem using Rewriting Logic, starting with a simple and elegant declarative model, whose correctness (in terms of schedule's optimality) is self-evident. We then refine this specification, inspired by the design of our specialised algorithm, to obtain an efficient system that can be used as a playground to explore various aspects of attack-defence trees. We compare the two approaches on different benchmarks.

==> benchmark.tex <==
\begin{tabular}{lrr}
  \toprule
  model                    & mean\_adt2amas & mean\_adt2maude \\
  \midrule
  forestall                & 20.05          & 160.12          \\
  gain\_admin              & 3342045.64     & 6129.03         \\
  icfem2020                & 2.51           & 180.35          \\
  interrupted              & 1.31           & 121.70          \\
  iot\_dev                 & 2652.56        & 629.17          \\
  last                     & 1.83           & 129.84          \\
  lukasz\_or               & 3.32           & 2352.39         \\
  lukasz                   & 54.48          & 140.74          \\
  scaling                  & 1.22           & 122.94          \\
  treasure\_hunters        & 26.70          & 131.56          \\
  adtree-d2\_w10\_c10\_AND & 6.24           & 211.55          \\
  adtree-d2\_w10\_c2\_AND  & 2.18           & 121.02          \\
  adtree-d2\_w10\_c4\_AND  & 4.82           & 174.60          \\
  adtree-d2\_w10\_c6\_AND  & 5.09           & 195.25          \\
  adtree-d2\_w10\_c8\_AND  & 8.51           & 367.50          \\
  adtree-d2\_w2\_c10\_AND  & 4.65           & 460.99          \\
  adtree-d2\_w2\_c2\_AND   & 1.71           & 119.65          \\
  adtree-d2\_w2\_c4\_AND   & 2.28           & 126.74          \\
  adtree-d2\_w2\_c6\_AND   & 2.56           & 157.62          \\
  adtree-d2\_w2\_c8\_AND   & 3.84           & 257.17          \\
  adtree-d2\_w3\_c10\_AND  & 4.65           & 517.66          \\
  adtree-d2\_w3\_c2\_AND   & 1.80           & 122.18          \\
  adtree-d2\_w3\_c4\_AND   & 1.92           & 125.45          \\
  adtree-d2\_w3\_c6\_AND   & 2.63           & 161.32          \\
  adtree-d2\_w3\_c8\_AND   & 3.34           & 277.93          \\
  adtree-d2\_w4\_c10\_AND  & 5.21           & 390.38          \\
  adtree-d2\_w4\_c2\_AND   & 1.75           & 121.00          \\
  adtree-d2\_w4\_c4\_AND   & 1.95           & 124.86          \\
  adtree-d2\_w4\_c6\_AND   & 2.86           & 149.19          \\
  adtree-d2\_w4\_c8\_AND   & 3.74           & 234.41          \\
  adtree-d2\_w5\_c10\_AND  & 5.82           & 323.08          \\
  adtree-d2\_w5\_c2\_AND   & 1.98           & 121.50          \\
  adtree-d2\_w5\_c4\_AND   & 3.17           & 144.32          \\
  adtree-d2\_w5\_c6\_AND   & 2.76           & 139.97          \\
  adtree-d2\_w5\_c8\_AND   & 3.56           & 202.94          \\
  adtree-d2\_w6\_c10\_AND  & 5.02           & 271.23          \\
  adtree-d2\_w6\_c2\_AND   & 2.12           & 120.33          \\
  adtree-d2\_w6\_c4\_AND   & 3.14           & 143.69          \\
  adtree-d2\_w6\_c6\_AND   & 3.00           & 139.67          \\
  adtree-d2\_w6\_c8\_AND   & 4.67           & 200.58          \\
  adtree-d2\_w7\_c10\_AND  & 5.03           & 263.66          \\
  adtree-d2\_w7\_c2\_AND   & 2.15           & 121.02          \\
  adtree-d2\_w7\_c4\_AND   & 3.06           & 140.16          \\
  adtree-d2\_w7\_c6\_AND   & 5.04           & 234.72          \\
  adtree-d2\_w7\_c8\_AND   & 4.02           & 173.29          \\
  adtree-d2\_w8\_c10\_AND  & 5.87           & 257.61          \\
  adtree-d2\_w8\_c2\_AND   & 2.33           & 120.87          \\
  adtree-d2\_w8\_c4\_AND   & 3.31           & 140.47          \\
  adtree-d2\_w8\_c6\_AND   & 5.29           & 201.85          \\
  adtree-d2\_w8\_c8\_AND   & 3.77           & 171.71          \\
  adtree-d2\_w9\_c10\_AND  & 6.17           & 215.26          \\
  adtree-d2\_w9\_c2\_AND   & 2.23           & 120.81          \\
  adtree-d2\_w9\_c4\_AND   & 4.55           & 175.83          \\
  adtree-d2\_w9\_c6\_AND   & 5.02           & 197.02          \\
  adtree-d2\_w9\_c8\_AND   & 6.85           & 381.88          \\
  adtree-d3\_w10\_c10\_AND & 7.87           & 508.73          \\
  adtree-d3\_w10\_c2\_AND  & 3.90           & 139.02          \\
  adtree-d3\_w10\_c4\_AND  & 6.28           & 241.56          \\
  adtree-d3\_w10\_c6\_AND  & 7.52           & 308.46          \\
  adtree-d3\_w10\_c8\_AND  & 10.80          & 738.69          \\
  adtree-d3\_w2\_c10\_AND  & 6.92           & 1139.06         \\
  adtree-d3\_w2\_c2\_AND   & 2.11           & 120.74          \\
  adtree-d3\_w2\_c4\_AND   & 2.23           & 141.90          \\
  adtree-d3\_w2\_c6\_AND   & 3.36           & 247.90          \\
  adtree-d3\_w2\_c8\_AND   & 4.86           & 545.92          \\
  adtree-d3\_w3\_c10\_AND  & 6.51           & 1512.87         \\
  adtree-d3\_w3\_c2\_AND   & 2.46           & 125.27          \\
  adtree-d3\_w3\_c4\_AND   & 2.70           & 146.08          \\
  adtree-d3\_w3\_c6\_AND   & 3.61           & 272.62          \\
  adtree-d3\_w3\_c8\_AND   & 5.22           & 702.80          \\
  adtree-d3\_w4\_c10\_AND  & 6.94           & 1104.14         \\
  adtree-d3\_w4\_c2\_AND   & 2.12           & 122.68          \\
  adtree-d3\_w4\_c4\_AND   & 2.57           & 137.63          \\
  adtree-d3\_w4\_c6\_AND   & 3.45           & 231.44          \\
  adtree-d3\_w4\_c8\_AND   & 5.16           & 547.68          \\
  adtree-d3\_w5\_c10\_AND  & 8.84           & 878.86          \\
  adtree-d3\_w5\_c2\_AND   & 2.66           & 136.90          \\
  adtree-d3\_w5\_c4\_AND   & 3.73           & 207.99          \\
  adtree-d3\_w5\_c6\_AND   & 3.74           & 221.63          \\
  adtree-d3\_w5\_c8\_AND   & 5.95           & 448.95          \\
  adtree-d3\_w6\_c10\_AND  & 7.52           & 707.68          \\
  adtree-d3\_w6\_c2\_AND   & 2.93           & 136.10          \\
  adtree-d3\_w6\_c4\_AND   & 3.50           & 182.51          \\
  adtree-d3\_w6\_c6\_AND   & 3.98           & 215.37          \\
  adtree-d3\_w6\_c8\_AND   & 5.62           & 369.80          \\
  adtree-d3\_w7\_c10\_AND  & 9.56           & 669.49          \\
  adtree-d3\_w7\_c2\_AND   & 3.44           & 150.79          \\
  adtree-d3\_w7\_c4\_AND   & 3.81           & 179.93          \\
  adtree-d3\_w7\_c6\_AND   & 6.23           & 411.91          \\
  adtree-d3\_w7\_c8\_AND   & 5.66           & 354.02          \\
  adtree-d3\_w8\_c10\_AND  & 7.76           & 541.62          \\
  adtree-d3\_w8\_c2\_AND   & 3.48           & 149.63          \\
  adtree-d3\_w8\_c4\_AND   & 3.57           & 175.13          \\
  adtree-d3\_w8\_c6\_AND   & 6.36           & 393.76          \\
  adtree-d3\_w8\_c8\_AND   & 5.90           & 346.68          \\
  adtree-d3\_w9\_c10\_AND  & 7.80           & 519.93          \\
  adtree-d3\_w9\_c2\_AND   & 4.66           & 150.04          \\
  adtree-d3\_w9\_c4\_AND   & 5.52           & 245.54          \\
  adtree-d3\_w9\_c6\_AND   & 6.81           & 382.09          \\
  adtree-d3\_w9\_c8\_AND   & 9.99           & 764.22          \\
  adtree-d4\_w10\_c10\_AND & 12.28          & 998.36          \\
  adtree-d4\_w10\_c2\_AND  & 5.92           & 248.09          \\
  adtree-d4\_w10\_c4\_AND  & 6.52           & 350.12          \\
  adtree-d4\_w10\_c6\_AND  & 9.65           & 636.92          \\
  adtree-d4\_w10\_c8\_AND  & 13.84          & 1372.79         \\
  adtree-d4\_w2\_c10\_AND  & 7.84           & 2402.93         \\
  adtree-d4\_w2\_c2\_AND   & 2.10           & 123.06          \\
  adtree-d4\_w2\_c4\_AND   & 2.66           & 178.86          \\
  adtree-d4\_w2\_c6\_AND   & 4.46           & 418.62          \\
  adtree-d4\_w2\_c8\_AND   & 6.19           & 1089.93         \\
  adtree-d4\_w3\_c10\_AND  & 8.87           & 3639.44         \\
  adtree-d4\_w3\_c2\_AND   & 2.42           & 130.85          \\
  adtree-d4\_w3\_c4\_AND   & 3.44           & 193.27          \\
  adtree-d4\_w3\_c6\_AND   & 4.15           & 497.47          \\
  adtree-d4\_w3\_c8\_AND   & 6.80           & 1482.87         \\
  adtree-d4\_w4\_c10\_AND  & 10.62          & 2419.35         \\
  adtree-d4\_w4\_c2\_AND   & 2.68           & 126.38          \\
  adtree-d4\_w4\_c4\_AND   & 2.83           & 169.30          \\
  adtree-d4\_w4\_c6\_AND   & 4.86           & 453.03          \\
  adtree-d4\_w4\_c8\_AND   & 8.40           & 1107.62         \\
  adtree-d4\_w5\_c10\_AND  & 10.79          & 2117.04         \\
  adtree-d4\_w5\_c2\_AND   & 3.82           & 149.45          \\
  adtree-d4\_w5\_c4\_AND   & 4.87           & 311.49          \\
  adtree-d4\_w5\_c6\_AND   & 4.49           & 366.74          \\
  adtree-d4\_w5\_c8\_AND   & 7.44           & 873.78          \\
  adtree-d4\_w6\_c10\_AND  & 14.07          & 1730.55         \\
  adtree-d4\_w6\_c2\_AND   & 3.50           & 147.54          \\
  adtree-d4\_w6\_c4\_AND   & 4.15           & 256.31          \\
  adtree-d4\_w6\_c6\_AND   & 4.55           & 353.16          \\
  adtree-d4\_w6\_c8\_AND   & 8.10           & 830.13          \\
  adtree-d4\_w7\_c10\_AND  & 11.63          & 1388.53         \\
  adtree-d4\_w7\_c2\_AND   & 4.14           & 169.05          \\
  adtree-d4\_w7\_c4\_AND   & 4.83           & 244.74          \\
  adtree-d4\_w7\_c6\_AND   & 8.47           & 724.80          \\
  adtree-d4\_w7\_c8\_AND   & 8.51           & 796.63          \\
  adtree-d4\_w8\_c10\_AND  & 11.22          & 1337.03         \\
  adtree-d4\_w8\_c2\_AND   & 3.86           & 167.25          \\
  adtree-d4\_w8\_c4\_AND   & 4.49           & 240.35          \\
  adtree-d4\_w8\_c6\_AND   & 8.34           & 683.84          \\
  adtree-d4\_w8\_c8\_AND   & 8.36           & 629.91          \\
  adtree-d4\_w9\_c10\_AND  & 15.51          & 1277.71         \\
  adtree-d4\_w9\_c2\_AND   & 6.52           & 252.64          \\
  adtree-d4\_w9\_c4\_AND   & 6.44           & 359.32          \\
  adtree-d4\_w9\_c6\_AND   & 8.37           & 661.51          \\
  adtree-d4\_w9\_c8\_AND   & 17.45          & 1701.17         \\
  adtree-d5\_w10\_c10\_AND & 16.10          & 2242.22         \\
  adtree-d5\_w10\_c2\_AND  & 7.10           & 311.11          \\
  adtree-d5\_w10\_c4\_AND  & 7.82           & 510.42          \\
  adtree-d5\_w10\_c6\_AND  & 10.98          & 1046.39         \\
  adtree-d5\_w10\_c8\_AND  & 16.24          & 2850.61         \\
  adtree-d5\_w2\_c10\_AND  & 11.53          & 4395.15         \\
  adtree-d5\_w2\_c2\_AND   & 3.46           & 126.42          \\
  adtree-d5\_w2\_c4\_AND   & 3.46           & 237.42          \\
  adtree-d5\_w2\_c6\_AND   & 4.66           & 703.38          \\
  adtree-d5\_w2\_c8\_AND   & 7.73           & 1963.23         \\
  adtree-d5\_w3\_c10\_AND  & 12.41          & 7007.98         \\
  adtree-d5\_w3\_c2\_AND   & 2.65           & 138.70          \\
  adtree-d5\_w3\_c4\_AND   & 3.30           & 279.66          \\
  adtree-d5\_w3\_c6\_AND   & 5.56           & 978.56          \\
  adtree-d5\_w3\_c8\_AND   & 8.95           & 2750.91         \\
  adtree-d5\_w4\_c10\_AND  & 13.72          & 5008.19         \\
  adtree-d5\_w4\_c2\_AND   & 2.51           & 130.78          \\
  adtree-d5\_w4\_c4\_AND   & 3.88           & 265.14          \\
  adtree-d5\_w4\_c6\_AND   & 4.94           & 766.37          \\
  adtree-d5\_w4\_c8\_AND   & 7.13           & 2013.91         \\
  adtree-d5\_w5\_c10\_AND  & 14.75          & 3955.27         \\
  adtree-d5\_w5\_c2\_AND   & 3.49           & 165.08          \\
  adtree-d5\_w5\_c4\_AND   & 4.42           & 479.84          \\
  adtree-d5\_w5\_c6\_AND   & 7.11           & 716.20          \\
  adtree-d5\_w5\_c8\_AND   & 10.37          & 1832.95         \\
  adtree-d5\_w6\_c10\_AND  & 15.19          & 3151.83         \\
  adtree-d5\_w6\_c2\_AND   & 3.30           & 162.42          \\
  adtree-d5\_w6\_c4\_AND   & 6.02           & 455.70          \\
  adtree-d5\_w6\_c6\_AND   & 5.75           & 562.72          \\
  adtree-d5\_w6\_c8\_AND   & 11.41          & 1479.24         \\
  adtree-d5\_w7\_c10\_AND  & 15.18          & 3012.90         \\
  adtree-d5\_w7\_c2\_AND   & 4.42           & 200.86          \\
  adtree-d5\_w7\_c4\_AND   & 5.27           & 352.64          \\
  adtree-d5\_w7\_c6\_AND   & 10.67          & 1447.54         \\
  adtree-d5\_w7\_c8\_AND   & 11.73          & 1397.10         \\
  adtree-d5\_w8\_c10\_AND  & 21.26          & 2913.02         \\
  adtree-d5\_w8\_c2\_AND   & 4.25           & 194.96          \\
  adtree-d5\_w8\_c4\_AND   & 5.07           & 340.28          \\
  adtree-d5\_w8\_c6\_AND   & 11.08          & 1143.81         \\
  adtree-d5\_w8\_c8\_AND   & 12.78          & 1349.00         \\
  adtree-d5\_w9\_c10\_AND  & 16.07          & 2319.45         \\
  adtree-d5\_w9\_c2\_AND   & 6.51           & 320.76          \\
  adtree-d5\_w9\_c4\_AND   & 8.54           & 529.97          \\
  adtree-d5\_w9\_c6\_AND   & 10.87          & 1093.02         \\
  adtree-d5\_w9\_c8\_AND   & 16.10          & 2953.78         \\
  \bottomrule
\end{tabular}


==> examples/interrupted.tex <==
%!TEX root=../main.tex

\begin{figure}
  \centering
  \begin{tikzpicture}
    \node at (0,0)   {\picADT{ADTree_interrupted.tikz}};
    \node at (4.5,0) {\picTable{tabAttributes_interrupted}};
  \end{tikzpicture}
  \caption{Interrupted schedule example}
  \label{fig:interrupted}
\end{figure}


